Epi-Convergence of Expectation Functions under Varying Measures and Integrands

For expectation functions on metric spaces, we provide sufficient conditions for epi-convergence under varying probability measures and integrands, and examine applications in the area of sieve estimators, mollifier smoothing, PDE-constrained optimization, and stochastic optimization with expectation constraints. As a stepping stone to epi-convergence of independent interest, we develop parametric Fatou's lemmas under mild integrability assumptions. In the setting of Suslin metric spaces, the assumptions are expressed in terms of Pasch-Hausdorff envelopes. For general metric spaces, the assumptions shift to semicontinuity of integrands also on the sample space, which then is assumed to be a metric space.

==> mac.tex <==
% January 7, 2008 (Monday, 21:17 PST) rjbw

\usepackage{theorem}
\usepackage{enumerate}
\usepackage{array}
\usepackage[reqno]{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{latexsym}
\usepackage{makeidx}
%% \usepackage{showidx}
\usepackage{fancybox}
\input epsf.sty
\usepackage[dvips]{graphicx,color}
\usepackage{showlabels}
\usepackage{subcaption}


\newcommand{\drawing}[4]{
	\begin{figure}[!hbt]
	\begin{center}
	\leavevmode
	\epsfxsize=#2
	\epsfbox{#1}
	\caption{\small #3}
	\label{#4}
	\end{center}
	\end{figure}}

% the proclaim commands
\theoremstyle{change}
\newtheorem{proclaim}{PROCLAIM}[section]
\newtheorem{theorem}[proclaim]{Theorem}
\newtheorem{definition}[proclaim]{Definition}
\newtheorem{lemma}[proclaim]{Lemma}
\newtheorem{proposition}[proclaim]{Proposition}
\newtheorem{corollary}[proclaim]{Corollary}
\newtheorem{example}[proclaim]{Example}
\newtheorem{exercise}[proclaim]{Exercise}
\newtheorem{convergence}[proclaim]{Convergence}
\newtheorem{algorithm}[proclaim]{Algorithm}
\newtheorem{assumption}[proclaim]{Assumption}
\newtheorem{remark}[proclaim]{Remark}
\newtheorem{interlude}[proclaim]{Interlude}

% proclaim labeling with marginal note
\newcommand{\rwlabel}[1]{\label{#1}\marginpar{#1}}

% numbering of equations
\numberwithin{equation}{section}

% \renewcommand{\thefootnote}{\fnsymbol{footnote}}

%formatting
% \newcommand{\beginsection}[1]{\bigskip\noindent{\bf #1}
%                   \medskip\vskip0pt\noindent\hskip0pt}
\outer\def\proclaim #1. #2\par{\medbreak \noindent{\bf#1.\enspace}{\sl#2}\par
  \ifdim\lastskip<\medskipamount
  \removelastskip\penalty55\medskip\fi}
\def\state #1. { \noindent{\bf#1.\enspace}}
\def\algo #1. { \noindent{\bf#1.\enspace}}
\newcommand{\newpar}{\vskip0cm\indent}
\newcommand{\head}[1]{\nopagenumbers\centerline{\bf #1}\bigskip}
\newcommand{\headskip}[1]{\null\vskip#1}
\newcommand{\paritem}[1]{\vskip0cm\noindent\hskip12pt{{\rm #1}}\hskip5pt}
\newcommand{\bigbar}{\vskip8pt\centerline{\hrulefill}\vskip8pt}
\newcommand{\rwtxt}[1]{\,\;\text{#1}\;\,}
\newcommand{\Text}[1]{\,\quad\hbox{#1}\quad\,}
\newcommand{\iitem}[2]{\everypar{\hangafter=1 \hangindent=16pt}
  \par\noindent\hskip8pt{#1}\hskip4pt #2 \everypar{\hangafter=0}}
\newcommand{\n}[2]{\par\noindent{\hangindent=25pt{\bf#1}\qd#2
     \par}\smallskip}
\newcommand{\nn}[2]{\par\noindent{\leftskip=15pt\hangindent=25pt{\bf#1}\qd#2
     \par}\smallskip}

%clusters
\DeclareMathOperator{\aff}{aff}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\minimax}{minimax}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\bdry}{bdry}
\DeclareMathOperator{\con}{con}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\nullspace}{null}
\DeclareMathOperator{\haus}{haus}
\DeclareMathOperator{\exs}{exs}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\gph}{gph}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\hypo}{hypo}
\DeclareMathOperator{\nt}{int}
\DeclareMathOperator{\lev}{lev}
\DeclareMathOperator{\lip}{lip}
\DeclareMathOperator{\pol}{pol}
\DeclareMathOperator{\pos}{pos}
\DeclareMathOperator{\prj}{prj}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rge}{rge}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\lsc}{lsc}
\DeclareMathOperator{\fcns}{fcns}
\DeclareMathOperator{\maps}{maps}
\DeclareMathOperator{\lscfcns}{lsc-fcns}
\DeclareMathOperator{\scfcns}{sc-fcns}
\DeclareMathOperator{\clfcns}{cl-fcns}
\DeclareMathOperator{\uscfcns}{usc-fcns}
\newcommand{\uscfcnsp}{\mathop{\textrm{usc-fcns}_+}}
\DeclareMathOperator{\ctsfcns}{cts-fcns}
\DeclareMathOperator{\bprob}{b-prob}
\DeclareMathOperator{\srsk}{s-rsk}
\DeclareMathOperator{\clsets}{cl-sets}
\DeclareMathOperator{\sets}{sets}
\DeclareMathOperator{\cvxfcns}{cvx-fcns}
\DeclareMathOperator{\acfcns}{ac-fcns}
\DeclareMathOperator{\pcfcns}{pc-fcns}
\DeclareMathOperator{\gap}{gap}
\DeclareMathOperator{\prx}{prx}
\DeclareMathOperator{\env}{env}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\biv}{\mathop{\rm biv}}
\DeclareMathOperator{\trc}{trc}
\newcommand{\lscbfcns}{\mathop{\textrm{lsc-bfcns}}}


\newcommand{\comp}{\,{\raise 1pt \hbox{$\scriptstyle\circ$}}\,}
\newcommand{\eqhyph}{\hbox{\rm -}}

%other symbols
%\newcommand{\reals}{{I\kern-.35em R}}
%\newcommand{\Reals}{\overline{I\kern-.35em R}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\Reals}{\overline{\mathbb{R}}}
\newcommand{\natnums}{{{\rm l} \kern -.13em {\rm N} }}
%\newcommand{\nats}{{I\kern -.35em N}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\snats}{{I\kern -.29em N}}
\newcommand{\rats}{{Q\kern -.64em \raise 1pt \hbox{$\scriptstyle |$}\;\,}}
\newcommand{\srats}
	{{Q\kern -.56em \raise 1.2pt \hbox{$\scriptscriptstyle /$}\,}}
\newcommand{\ints}{Z\kern -.46em Z}
%\newcommand{\ball}{{I\kern -.35em B}}
\newcommand{\ball}{\mathbb{B}}
\newcommand{\pluss}{\hskip1pt \raise1pt\vbox{\hrule width6pt \vskip1pt \hrule
                    width6pt} \kern-4pt{\lower1pt\hbox{\vrule height6pt
		    \kern1pt\vrule height6pt}}\hskip5pt}
\newcommand{\eop}
	{\hfill{$\vcenter{\hrule height1pt \hbox{\vrule width1pt height5pt
   	 \kern5pt \vrule width1pt} \hrule height1pt}$} \medskip}
\newcommand{\half}
	{{\raisebox{1pt}{$\frac{1}{2}$}}}
\newcommand{\third}
	{{\raisebox{1pt}{$\frac{1}{3}$}}}
\newcommand{\fourthird}
	{{\raisebox{1pt}{$\frac{4}{3}$}}}
\newcommand{\ninth}
	{{\raisebox{1pt}{$\frac{1}{9}$}}}
\newcommand{\twoninth}
	{{\raisebox{1pt}{$\frac{2}{9}$}}}
\newcommand{\twothird}
	{{\raisebox{1pt}{$\frac{2}{3}$}}}
\newcommand{\proxfac}
	{{\raisebox{1pt}{$\frac{1}{2\lambda}$}}}
\newcommand{\proxfacnuone}
	{{\raisebox{1pt}{$\frac{1}{2\lambda_1^\nu}$}}}
\newcommand{\proxfacnutwo}
	{{\raisebox{1pt}{$\frac{1}{2\lambda_2^\nu}$}}}
\newcommand{\proxfacnu}
	{{\raisebox{1pt}{$\frac{1}{2\lambda^\nu}$}}}
\newcommand{\tproxfac}
	{{\raisebox{1pt}{$\frac{1}{\lambda}$}}}
\newcommand{\tproxfacnu}
	{{\raisebox{1pt}{$\frac{1}{\lambda^\nu}$}}}
\newcommand{\overlamrho}
	{{\raisebox{1pt}{$\frac{1}{\lambda\rho}$}}}
\newcommand{\linfty}{{\scriptscriptstyle \infty}}
\newcommand{\lminus}{{\scriptscriptstyle -}}
\newcommand{\lplus}{{\scriptscriptstyle +}}
\newcommand{\lT}{{\scriptscriptstyle T}}
\newcommand{\mvert}{{\,\big\vert\,}}
\newcommand{\bull}{\hbox{$\,\bullet\,$}}
\newcommand{\setd}{{ d \kern -.15em l}}
\newcommand{\hatsetd}{ d \hat{\kern -.15em l }}
\newcommand{\hatsetde}{d\!\hat l^{\rm e}}
\newcommand{\hatsetdd}{d\!\hat l^{\delta}}
\newcommand{\hatsetdnull}{d\!\hat l^0}

%greek symbols
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}

% delimiters
\newcommand{\lset}{\big\lbrace}
\newcommand{\mset}{{\,\big\vert\,}}
\newcommand{\rset}{\big\rbrace}
\newcommand{\Lset}{\Big\lbrace}
\newcommand{\Mset}{{\,\Big\vert\,}}
\newcommand{\Rset}{\Big\rbrace}
\newcommand{\Langle}{\Big\langle}
\newcommand{\Rangle}{\Big\rangle}
\newcommand{\Leq}{\;\leq\;}
\newcommand{\Geq}{\;\geq\;}

%miscellaneous hyphenation
\hyphenation{sto-chast-ic}
\hyphenation{semi-def-i-nite}
\hyphenation{La-gran-gi-an}
\hyphenation{non-smooth}
\hyphenation{sub-diffe-ren-tial}
\hyphenation{inf--pro-jec-tion}
\hyphenation{epi-poly-he-dral}

% Arrows:
\newcommand{\tto}{\;{\lower 1pt \hbox{$\rightarrow$}}\kern -12pt
           \hbox{\raise 2.5pt \hbox{$\rightarrow$}}\;}
\newcommand{\overto}[1]{\,{\raise 0pt\hbox{$\rightarrow$}}\kern -9pt
     \hbox{\lower 3pt \hbox{$\scriptscriptstyle#1$}}\hskip6pt}
\newcommand{\underto}[1]{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -9pt
     \hbox{\raise 4pt \hbox{$\,\scriptscriptstyle#1$}}\hskip7pt}
\newcommand{\bigoverto}[1]{{\raise 0pt\hbox{$\,\longrightarrow$}}\kern -16pt
     \hbox{\lower 3pt \hbox{$\scriptscriptstyle#1$}}\hskip4pt}
\newcommand{\bigunderto}[1]{\,{\lower 1pt\hbox{$\longrightarrow$}}\kern -16pt
     \hbox{\raise 4pt \hbox{$\,\scriptscriptstyle#1$}}\hskip6pt}
\newcommand{\bigbigto}[2]{\,{\raise 0pt\hbox{$\,\longrightarrow$}}\kern -16pt
     \hbox{\lower 3pt \hbox{$\scriptscriptstyle#2$}}\kern -10pt
     \hbox{\raise 4pt \hbox{$\,\scriptscriptstyle#1$}}\hskip7pt}
\newcommand{\downto}{{\raise 1pt \hbox{$\scriptscriptstyle \,\searrow\,$}}}
\newcommand{\upto}{{\raise 1pt \hbox{$\scriptscriptstyle \,\nearrow\,$}}}
\newcommand{\imply}{\quad\hbox{$\Longrightarrow$}\quad}
% \newcommand{\implies}{\quad\hbox{$\Longrightarrow$}\quad}
\newcommand{\implied}{\quad\hbox{$\Longleftarrow$}\quad}
\newcommand{\notimply}
	{\quad\hbox{$\Longrightarrow \kern -14pt {/}$}\hskip6pt\quad}
% \newcommand{\iff}{\quad\hbox{$\Longleftrightarrow$}\quad}
% \newcommand{\rightrightarrows}{\,{{\lower4pt\hbox{$\scriptstyle\rightarrow$}}
    %\atop{\raise8pt\hbox{$\scriptstyle\rightarrow$}}}\,} %supplanted by \tto
\newcommand{\lrw}{\small{\leftrightarrow}}
\newcommand{\lseg}[2]{#1\!\leftrightarrow\!#2}
\newcommand{\lsego}[2]{#1\!\!\leftrightarrow\!\!#2}

\newcommand{\hlim}{{\mathop{\hbox{\rm e-lim}}}}
\newcommand{\lto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4pt \hbox{$\, \scriptstyle l$}}\hskip7pt}
\newcommand{\eto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4pt \hbox{$\, \scriptstyle e$}}\hskip7pt}
\newcommand{\hto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4pt \hbox{$\, \scriptstyle h$}}\hskip7pt}
\newcommand{\pto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4.5pt \hbox{$\, \scriptstyle p$}}\hskip7pt}
\newcommand{\cto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4pt \hbox{$\, \scriptstyle c$}}\hskip7pt}
\newcommand{\gto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4.5pt \hbox{$\, \scriptstyle g$}}\hskip7pt}
\newcommand{\sto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -10pt
     \hbox{\raise 4pt \hbox{$\, \scriptstyle s$}}\hskip7pt}
\newcommand{\awto}{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -15pt
     \hbox{\raise 4pt \hbox{$\, \scriptstyle aw$}}\hskip7pt}
%\def\Nto{\,{\lower 1pt\hbox{$\rightarrow$}}\kern -12pt
%     \hbox{\raise 4pt \hbox{$\, \scriptstyle N$}}\hskip7pt}
\def\Nto{\,{\raise 1pt\hbox{$\rightarrow$}}\kern -13pt
     \hbox{\lower 3pt \hbox{$\, \scriptstyle N$}}\hskip7pt}
\def\Cto{\,{\raise 1pt\hbox{$\rightarrow$}}\kern -14pt
     \hbox{\lower 3pt \hbox{$\, \scriptstyle C$}}\hskip7pt}
\def\fto{\,{\raise 1pt\hbox{$\rightarrow$}}\kern -14pt
     \hbox{\lower 3pt \hbox{$\, \scriptstyle f$}}\hskip7pt}


% vertical adjustments:
% \newcommand{\substack}[2]{{\scriptstyle{#1}\atop\scriptstyle{#2}}}
\newcommand{\subsubstack}[3]{ {{\scriptstyle{#1}}\atop{ \scriptstyle{#2}}}
                   \atop{\scriptstyle{#3}} }
\newcommand{\vinf}{\mathop{\smash\inf\vphantom\sup}}
\newcommand{\vlim}{\mathop{\smash\lim\vphantom\sup}}
\newcommand{\vliminf}{\mathop{\smash\liminf\vphantom\limsup}}
\newcommand{\vmax}{\mathop{\smash\max\vphantom\sup}}
\newcommand{\vmin}{\mathop{\smash\min\vphantom\sup}}
\newcommand{\vsup}{\mathop{\smash\sup\vphantom\sup}}
\newcommand{\low}[1]{{\lower1pt \hbox{$\scriptstyle #1$}}}
\newcommand{\loww}[1]{{\lower2pt \hbox{$\scriptstyle #1$}}}
\newcommand{\high}[1]{{\raise1pt \hbox{$\scriptstyle #1$}}}

% Script capitals:
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cE}{{\cal E}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cG}{{\cal G}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cJ}{{\cal J}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cQ}{{\cal Q}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cW}{{\cal W}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
\newcommand{\cZ}{{\cal Z}}

% broadened marks
% \newcommand{\Bar}{\overline}
%\newcommand{\Hat}{\widehat}
% \newcommand{\Tilde}{\widetilde}

%big union, intersection
\let\Cup=\bigcup
\let\Cap=\bigcap

% limits without limits
\newcommand{\nsum}{\mathop{\sum}\nolimits}
\newcommand{\nprod}{\mathop{\prod}\nolimits}
\newcommand{\nInnLim}{\mathop{\rm LimInn}\nolimits}
\newcommand{\nOutLim}{\mathop{\rm Lim\hspace{-0.01cm}Out}\nolimits}
\newcommand{\nLim}{\mathop{\rm Lim}\nolimits}
\newcommand{\nlev}{\mathop{\lev}\nolimits}
\newcommand{\nlim}{\mathop{\rm lim}\nolimits}
\newcommand{\nliminf}{\mathop{\rm liminf}\nolimits}
\renewcommand{\liminf}{\mathop{\rm liminf}}
\newcommand{\nlimsup}{\mathop{\rm limsup}\nolimits}
\newcommand{\ninf}{\mathop{\rm inf}\nolimits}
\newcommand{\nsup}{\mathop{\rm sup}\nolimits}
\newcommand{\nmax}{\mathop{\rm max}\nolimits}
\newcommand{\nmin}{\mathop{\rm min}\nolimits}
\newcommand{\nnmin}{\mathop{\rm minimize}}
\newcommand{\nnmax}{\mathop{\rm maximize}}
\newcommand{\miz}{\mathop{\rm minimize}}
\newcommand{\maz}{\mathop{\rm maximize}}
\newcommand{\nargmax}{\mathop{\rm argmax}\nolimits}
\newcommand{\nargmin}{\mathop{\rm argmin}\nolimits}

% Derivatives:
\newcommand{\dir}{\vec{d}}
\newcommand{\dil}{\bar{d}}
% \newcommand{\dil}{\overset{\text{\tiny$\leftrightarrow$}}{d}}
\newcommand{\der}{{\hbox{\sl d}}\hskip.5pt}
\newcommand{\dersq}{{\hbox{\sl d}}\hskip.5pt^2\hskip-1.1pt}
\newcommand{\coder}{\partial}
\newcommand{\subg}{\partial}
\newcommand{\rsubg}{\Hat\partial}
\newcommand{\lsubg}{\vec\partial}
\newcommand{\dder}{\vec\der}
% \newcommand{\rder}{\kern 3pt \hbox{$\Hat{\hbox{\kern -3pt \sl d}}$}}
% \newcommand{\lrder}{\kern 1pt \hbox{$\Hat{\hbox{\kern -1pt \sl d}}$}}  %for book notes
% \newcommand{\rcoder}{\Hat\partial} \newcommand{\rhcoder{\Hat\partial^{\raise
%                              1pt\hbox{$\scriptscriptstyle\infty$}}\!}

%probabilistic clusters
\newcommand{\diffsn}{\mathop{\sl diffsn}\nolimits}
\newcommand{\revert}{\mathop{\sl revert}\nolimits}
\newcommand{\cov}{{\mathop{\rm cov}\nolimits}}
\newcommand{\var}{{\mathop{\rm var}\nolimits}}
\newcommand{\std}{\hspace{0.04cm}{\mathop{\rm std}\nolimits}\hspace{-0.04cm}}
\newcommand{\prob}{{\mathop{\rm prob}\nolimits}}
\newcommand{\rsk}{{\mathop{\rm rsk}\nolimits}}
\newcommand{\dev}{{\mathop{\rm dev}\nolimits}}
\newcommand{\err}{{\mathop{\rm err}\nolimits}}
\newcommand{\reg}{{\mathop{\rm reg}\nolimits}}
\newcommand{\fcn}{{\mathop{\rm fcn}\nolimits}}
\newcommand{\stat}{{\mathop{\rm stat}\nolimits}}

% mathematical boldface
\newcommand{\bfxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bfeta}{\mbox{\boldmath $\eta$}}
\newcommand{\bfzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\bfrho}{\mbox{\boldmath $\rho$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bfbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bfGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bfeps}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bflambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bfpi}{\mbox{\boldmath $\pi$}}

\newcommand{\bfT}{\mbox{\boldmath $T$}}
\newcommand{\bfB}{\mbox{\boldmath $B$}}
\newcommand{\bfV}{\mbox{\boldmath $V$}}
\newcommand{\bft}{\mbox{\boldmath $t$}}
\newcommand{\bfa}{\mbox{\boldmath $a$}}
\newcommand{\bfb}{\mbox{\boldmath $b$}}
\newcommand{\bfd}{\mbox{\boldmath $d$}}
\newcommand{\bfy}{\mbox{\boldmath $y$}}
\newcommand{\bfr}{\mbox{\boldmath $r$}}
\newcommand{\bfs}{\mbox{\boldmath $s$}}
\newcommand{\bfS}{\mbox{\boldmath $S$}}
\newcommand{\bfz}{\mbox{\boldmath $z$}}
\newcommand{\bfv}{\mbox{\boldmath $v$}}
\newcommand{\bfw}{\mbox{\boldmath $w$}}
\newcommand{\bfx}{\mbox{\boldmath $x$}}
\newcommand{\bfG}{\mbox{\boldmath $G$}}
\newcommand{\bfnull}{\mbox{\boldmath $0$}}
\newcommand{\bfone}{\mbox{\boldmath $1$}}

% new, germane to STO.PROG.
\newcommand{\sothat}{\mathop{\rm subject\; to\;}\nolimits}
\newcommand{\suchthat}{\mathop{\rm \;such\; that\;}\nolimits}

\newcommand{\lwdy}[2]{\mathrel{\mathop
        {\raisebox{0.1ex}{\null$#1$}}{\hbox{\kern -1.0em
	{\raisebox{-0.8ex}{$\scriptstyle{\;\to #2}$}}}}}}
\newcommand{\lwwdy}[2]{\mathrel{\mathop
        {\raisebox{0.2ex}{\null$#1$}}{\hbox{\kern -1.0em
	{\raisebox{-1.1ex}{$\scriptstyle{\;\to #2}$}}}}}}
\newcommand{\slwdy}[2]{\scriptsize{{\mathrel{\mathop
        {\raisebox{0.1ex}{\null$#1$}}{\hbox{\kern -1.0em
	{\raisebox{-0.8ex}{$\scriptstyle{\;\to #2}$}}}}}}}}
\newcommand{\slwwdy}[2]{\scriptsize{{\mathrel{\mathop
        {\raisebox{0.2ex}{\null$#1$}}{\hbox{\kern -1.0em
	{\raisebox{-1.1ex}{$\scriptstyle{\;\to #2}$}}}}}}}}
\newcommand{\cc}{\!:}
\newcommand{\ts}{\thinspace}

% colors
\definecolor{lightgray}{gray}{0.75}
\definecolor{myred}{rgb}{0.55,0,0}
\definecolor{myblue}{rgb}{0,0,0.5} % hex: #00007f
\definecolor{mygreen}{rgb}{0,0.5,0} % hex: #00007f
\definecolor{purple}{rgb}{0.5,0,0.5} % hex: #00007f
\definecolor{turq}{rgb}{0,0.805,0.816} % hex: #00007f
\definecolor{maroon}{rgb}{0.51,0,0}
\definecolor{MAROON}{rgb}{0.51,0,0}
\definecolor{redor}{rgb}{0.78,0.078,0.078}
\definecolor{dgreen}{rgb}{0,0.3,0}
%% \definecolor{dgreen}{rgb}{0,0.2,0}
\newcommand{\rxi}{{\textcolor{dgreen}{$\bfxi$}}}

% colors
\newcommand{\blue}{\color{blue}}
\newcommand{\brown}{\color{brown}}
\newcommand{\orange}{\color{orange}}
\newcommand{\black}{\color{black}}
\newcommand{\green}{\color{DarkGreen}}
\newcommand{\red}{\color{red}}
\newcommand{\purple}{\color{purple}}
\newcommand{\maroon}{\color{maroon}}
\newcommand{\MAROON}{\color{MAROON}}
\newcommand{\dgreen}{\color{dgreen}}

%% New 2017-2-1
%\newcommand{\Ex}{{I\kern-.36em E}}
\newcommand{\Ex}{\mathbb{E}}
\newcommand{\supquant}{\bar{\mathbb{Q}}}
\newcommand{\quant}{\mathbb{Q}}
\newcommand{\grill}{{\scriptscriptstyle\#}}
\newcommand{\bcdot}{\,{\raise .2ex \hbox{$\centerdot$}}\,}

% epi-splines
\newcommand{\diam}{\textup{\textrm{diam}}}
\newcommand{\poly}{\textup{\textrm{poly}}}
\newcommand{\espl}{\textup{\textrm{e-spl}}}
\newcommand{\rspl}{\textup{\textrm{r-spl}}}
\newcommand{\cspl}{\textup{\textrm{c-spl}}}
\newcommand{\xspl}{\textup{\textrm{x-spl}}}
\newcommand{\msh}{\textup{\textrm{msh}}}
\newcommand{\bfcns}{\mathop{\rm bfcns}}
\newcommand{\ninfsup}{\mathop{\rm infsup}\nolimits}
\newcommand{\nargminsup}{\mathop{\rm argminsup}\nolimits}


\newcommand{\lhyph}{\!\hbox{\rm -}\!}

% BlackboardBold Letters
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
% \newcommand{\syl}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

